Reduced Complexity Optimal Detection of Binary Faster-than-Nyquist Signaling

In this paper, we investigate the detection problem of binary faster-than-Nyquist (FTN) signaling and propose a novel sequence estimation technique that exploits its special structure. In particular, the proposed sequence estimation technique is based on sphere decoding (SD) and exploits the following two characteristics about the FTN detection problem: 1) the cor- relation between the noise samples after the receiver matched filter, and 2) the structure of the intersymbol interference (ISI) matrix. Simulation results show that the proposed SD-based sequence estimation (SDSE) achieves the optimal performance of the maximum likelihood sequence estimation (MLSE) at reduced computational complexity. This paper demonstrates that FTN signaling has the great potential of increasing the data rate and spectral efficiency substantially, when compared to Nyquist signaling, for the same bit-error-rate (BER) and signal-to-noise ratio (SNR).

==> SDR.tex <==
\section{Binary FTN signaling Detection using Proposed SDRSE} \label{sec:SDR}

%Despite the reduced number of arithmetic operations of the proposed SD equalizer, its worst case computation complexity still can be exponential. That said, in the following section, we propose a SDR based equalization technique with polynomial time worst case computational complexity. In this section, we introduce SDR based equalization technique to detect the binary FTN signaling in \eqref{eq:opML}.

Despite the reduced complexity of the proposed SDSE when compared to the standard SD algorithm, its worst time complexity is still exponential. In this section, we propose an SDRSE that approaches the performance of the SDSE at polynomial time complexity.
SDR is a powerful and computationally efficient approximation technique for solving classes of non-convex optimization problems \cite{luo2010semidefinite}, where it is very hard to obtain the global optimal solution. In addition, SDR solution has a proven approximation accuracy, when compared to the global solution, under different problem settings \cite{goemans1995improved} and even can achieve the global optimal solution if a number of conditions are satisfied \cite{ye2003new}. 
%In general, SDR provides accurate (and sometimes near-optimal solutions).
%Randomization plays an indispensable role in finding SDR solutions.

The objective function of the MLSE optimization problem $\mathcal{OP}_{\rm{MLSE}}$ to detect the binary FTN signaling in \eqref{eq:opML} can be simplified as
\begin{eqnarray}\label{eq:opEQ_0}
	(\bm{z} - \bm{a})^{\rm{T}}  \bm{G}  (\bm{z} - \bm{a}) &=& \bm{z}^{\rm{T}} \bm{G} \bm{z} - \bm{a}^{\rm{T}} \bm{G} \bm{z} - \bm{z}^{\rm{T}} \bm{G} \bm{a} + \bm{a}^{\rm{T}} \bm{G} \bm{a}\nonumber\\
	&=& \bm{z}^{\rm{T}} \bm{G} \bm{z} + \bm{a}^{\rm{T}} \bm{G} \bm{a} - 2 \bm{z}^{\rm{T}} \bm{G} \bm{a}\nonumber\\
	&=& \bm{z}^{\rm{T}} \bm{G} \bm{z} + \bm{a}^{\rm{T}} \bm{G} \bm{a} - 2 (\bm{G} \bm{z})^{\rm{T}} \bm{a} \nonumber\\
	&=& \bm{z}^{\rm{T}} \bm{G} \bm{z} + \bm{a}^{\rm{T}} \bm{G} \bm{a} - 2 \bm{y}^{\rm{T}} \bm{a}.
\end{eqnarray}
That said, $\mathcal{OP}_{\rm{MLSE}}$ in  \eqref{eq:opML} can be rewritten as
\begin{eqnarray}
\hat{\bm{a}}_{\rm{SDR}} &=& \arg \: \underset{\bm{a}}{\min} \quad \bm{a}^{\rm{T}} \bm{G}  \bm{a} - 2 \bm{y}^{\rm{T}} \bm{a}, \nonumber \\
	& & {\textup{subject to}} \qquad \bm{a} \in \{1 , -1\}^N. \label{eq:opEQ}
\end{eqnarray}
It is worthy to mention that the objective functions in \eqref{eq:opEQ_0} and \eqref{eq:opEQ} differ by a constant value, i.e. $\bm{z}^{\rm{T}} \bm{G} \bm{z}$, with respect to the optimization variable $\bm{a}$. This implies that the numerical values of the two objectives are different, but their optimal solutions are the same. The binary FTN signaling detection problem  in \eqref{eq:opEQ} is classified as an NP-hard nonconvex Boolean Quadratic Program (BQP)  that is well-known to be a computationally difficult problem \cite{Boyd2004convex}. Lower bounds on the optimal value of the objective function in \eqref{eq:opEQ} can be obtained by using the Lagrangian duality or semidefinite programming. In the following, we discuss how SDR can be used to obtain a \textit{good} estimate of the data symbols vector $\hat{\bm{a}}$ in the binary FTN detection problem  in \eqref{eq:opEQ}.

\subsection{SDR  Solution}

The first term of the objective function in \eqref{eq:opEQ} can be re-expressed as
\begin{eqnarray}
	\bm{a}^{\rm{T}}\bm{G} \bm{a} = \Tr\{\bm{a}^{\rm{T}} \bm{G} \bm{a}\} = \Tr\{\bm{G}  \bm{a} \bm{a}^{\rm{T}}\} = \Tr\{\bm{G} \bm{A}\},
\end{eqnarray}
where $\bm{A} = \bm{a} \bm{a}^{\rm{T}}$.  As such, an equivalent MLSE optimization problem to detect the binary FTN signaling to the problem  in \eqref{eq:opEQ} is rewritten as
\begin{eqnarray}\label{eq:opSD}
\underset{\bm{A} \: \in \: \mathbb{S}^N, \:\bm{a}  \: \in \: \{1,\: -1\}^N}{\min} & & \Tr\{\bm{G} \bm{A}\} + 2 \hat{\bm{y}}^{\rm{T}} \bm{a}, \nonumber \\
	%& & {\textup{subject to}} \qquad  A_{ii} = 1, \quad i = 1, ..., N, \nonumber \\
	{\textup{subject to}} & &   \diag\{\bm{A}\} = 1,  \nonumber \\
	& &  \bm{A} = \bm{a} \bm{a}^{\rm{T}},
\end{eqnarray}
where $\mathbb{S}^N$ denotes the set of all real symmetric $N \times N$ matrices and $\hat{\bm{y}} = - \bm{y}$. The new variable $\bm{A} = \bm{a} \bm{a}^{\rm{T}}$ is equivalent to the matrix $\bm{A}$ being a rank one symmetric positive semidefinite, i.e., $\rank\{\bm{A}\} = 1$ and $\bm{A} \succeq 0$. The objective function in \eqref{eq:opSD} is linear over the set of matrices $\bm{A}$ and data symbols vector $\bm{a}$ that lie in the positive semidefinite cone. The equivalent MLSE optimization problem to detect the binary FTN signaling in \eqref{eq:opSD}, like its counterpart in \eqref{eq:opEQ}, is still non-convex and hard to solve.
However, the reformulation from \eqref{eq:opEQ} to \eqref{eq:opSD} allows us to identify the fundamental difficulty in solving the original MLSE optimization problem to detect the binary FTN signaling. It is clear from \eqref{eq:opSD} that the difficulty lies in the nonconvex rank one constraint, i.e. $\bm{A} = \bm{a} \bm{a}^{\rm{T}}$. We relax this problem into a convex one by replacing the nonconvex rank one constraint with a convex positive semidefinite constraint $\bm{A} - \bm{a} \bm{a}^{\rm{T}} \succeq 0$. Such  relaxation  produces a lower bound on the optimal solution of the MLSE optimization problem to detect the binary FTN signaling  in \eqref{eq:opEQ}. Further, we substitute this positive semidefinite constraint, i.e., $\bm{A} - \bm{a} \bm{a}^{\rm{T}} \succeq 0$, with its Schur complement \cite{Boyd2004convex}. Hence, the detection problem of binary FTN signaling is written as 
\begin{eqnarray}\label{eq:opSDC}
\mathcal{OP}_{\rm{SDR}}: \quad \underset{\bm{A} \: \in \: \mathbb{S}^N, \: \bm{A} \: \succeq \: 0, \:\bm{a}  \: \in \: \{1, \: -1\}^N}{\min} & & \Tr\{\bm{G} \bm{A}\} + 2 \hat{\bm{y}}^{\rm{T}} \bm{a} \nonumber \\
	%& & {\textup{subject to}} \qquad  A_{ii} = 1, \quad i = 1, ..., N, \nonumber \\
	 {\textup{subject to}} & &  \diag\{\bm{A}\} = 1,  \nonumber \\
	& & \begin{bmatrix}
		\bm{A} & \bm{a}\\ 
		\bm{a}^{\rm{T}} & 1
	\end{bmatrix} \succeq 0.
\end{eqnarray}
The optimization problem in \eqref{eq:opSDC} is the SDR of $\mathcal{OP}_{\rm{MLSE}}$ in \eqref{eq:opML}, and it can be solved, to any arbitrary accuracy, in a numerically reliable and efficient fashion \cite{grant2010cvx}.

The question now is how to convert the global solution $\bm{A}^*$ of $\mathcal{OP}_{\rm{SDR}}$ in \eqref{eq:opSDC} into a feasible solution $\hat{\bm{a}}$  in the problem  in \eqref{eq:opEQ}. A number of methods exists that can do this; however, we emphasize that the outcomes of such methods will be feasible for the problem  in \eqref{eq:opEQ}, but in general they will not be the global  optimal solutions. This is intuitive as we would have solved an NP-hard problem in polynomial time complexity. In the following subsection we discuss one of the most effective techniques, i.e., randomization,  to obtain a feasible solution to the detection problem in \eqref{eq:opEQ} from the SDR solution $\bm{A}^*$.

%After solving \eqref{eq:opSDC}, we obtain the optimal solutions $\bm{A}^*$ and $\bm{a}^*$. However, due to the relaxation to the Schur complement constraint, $\bm{a}^*$ may not satisfy $\bm{a}^* \in \{-1, 1\}$\footnote{It is not expected that $\bm{a}^*$ satisfies this constraint, as we would have solved an NP-hard problem in a polynomial time complexity.}. 

\subsection{Randomization}
Gaussian randomization \cite{luo2010semidefinite} is a key method to estimate the data symbol vector $\hat{\bm{a}}$ that is good enough and satisfies the constraint that   $\hat{\bm{a}} \in \{-1, 1\}^N$. 
The $\mathcal{OP}_{\rm{SDR}}$ in \eqref{eq:opSDC} produces a positive semidefinite matrix $\bm{A}$ in addition to the lower bound on the objective value. Randomization method exploits such a positive semidefinite matrix to facilitate obtaining a good feasible solution to the original problem  in \eqref{eq:opEQ}.

The intuition behind Gaussian randomization is to solve a stochastic version of \eqref{eq:opSDC}, where the optimal solution $\bm{a}^*$ is considered as the mean of a multivariate Gaussian random vector with $\bm{A}^* - \bm{a}^* \bm{a}^{*\rm{T}}$ as its covariance matrix. This stochastic optimization problem is written as
\begin{eqnarray}
\underset{\mathbb{E}\{\bm{\xi} \bm{\xi}^{\rm{T}}\} = \Xi, \: \mathbb{E}\{\bm{\xi}\} = \bm{a}^*}{\min} & & \mathbb{E}_{\bm{\xi} \sim \mathcal{N}({\bm{a}^*}, \bm{A}^* - \bm{a}^* \bm{a}^{*\rm{T}})}\{\Tr\{\bm{G} \bm{\xi} \bm{\xi}^{\rm{T}}\} + 2 \hat{\bm{y}}^{\rm{T}} \bm{\xi}\} \nonumber \\
%& & {\textup{subject to}} \qquad  A_{ii} = 1, \quad i = 1, ..., N, \nonumber \\
 {\textup{subject to}} & &  \mathbb{E}_{\bm{\xi} \sim \mathcal{N}({\bm{a}^*}, \bm{A}^* - \bm{a}^* \bm{a}^{*\rm{T}})}\{\diag\{\bm{\bm{\xi} \bm{\xi}^{\rm{T}}}\}\} = 1,  \nonumber \\
 & & \mathbb{E}_{\bm{\xi} \sim \mathcal{N}({\bm{a}^*}, \bm{A}^* - \bm{a}^* \bm{a}^{*\rm{T}})}\left\{\begin{bmatrix}
\bm{\bm{\xi} \bm{\xi}^{\rm{T}}} & \bm{\xi}\\ 
\bm{\xi}^{\rm{T}} & 1
\end{bmatrix}\right\} \succeq 0,
\end{eqnarray}
where $\Xi = \begin{bmatrix}
\bm{\bm{\xi} \bm{\xi}^{\rm{T}}} & \bm{\xi}\\ 
\bm{\xi}^{\rm{T}} & 1
\end{bmatrix}$. Now, the estimated data symbols $\hat{\bm{a}}$ can be reached as follows.  We generate $\bm{\xi}_{q}$, $q = 1, ..., Q,$ where $Q$ is the total number of generated RVs as  $\bm{\xi}_{q} \sim (\bm{a}^*, \bm{A}^* - \bm{a}^* \bm{a}^{*\rm{T}})$, then the values of $\bm{\xi}_{q}$ is quantized as $\breve{\bm{a}}_{q} = {\rm{sgn}}\{{\bm{\xi}}_{q}\}$, where ${\rm{sgn}}$ is the sign function. Then the optimal value of $q$, i.e., $q^*$, that minimizes the objective function in   \eqref{eq:opEQ} can be written as

\begin{eqnarray}
	q^* & = & \arg \: \underset{q \:=\: 1, ..., Q}{\min} \quad {\breve{\bm{a}}_{q}}^{\rm{T}} \bm{G} \breve{\bm{a}}_{q} - 2 \bm{y}^{\rm{T}} \breve{\bm{a}}_{q},
\end{eqnarray}	
and finally the estimated data symbol can be calculated as
\begin{eqnarray}
	\hat{\bm{a}} & = & \breve{\bm{a}}_{q^*}.
\end{eqnarray}

The proposed SDRSE is formally expressed as follows:

{\textit{Algorithm 2:} Proposed SDRSE}
\begin{enumerate}
		\item \textbf{Input:} Pulse shape $p(t)$, received samples $\bm{y}$, and number of randomization iterations $Q$.
		\item Solve $\mathcal{OP}_{\rm{SDR}}$ in \eqref{eq:opSDC}  to find $\bm{A}^*$ and $\bm{a}^*$.
		\item Generate RV $\bm{\xi}_{q}$ as $\bm{\xi}_{q} \sim (\bm{a}^*, \bm{A}^* - \bm{a}^* \bm{a}^{*\rm{T}})$, $q = 1, ..., Q$.
		\item Find $\breve{\bm{a}}_{q} = {\rm{sgn}}\{{\bm{\xi}}_{q}\}$.
		\item Find $q^*  =  \arg \: \underset{q \:=\: 1, ..., Q}{\min} \quad {\breve{\bm{a}}_{q}}^{\rm{T}} \bm{G} \breve{\bm{a}}_{q} - 2 \bm{y}^{\rm{T}} \breve{\bm{a}}_{q}$.
		\item $\hat{\bm{a}} = \breve{\bm{a}}_{q^*}$.
		\item \textbf{Output:} Estimated data symbols $\hat{\bm{a}}_{\rm{SDR}}$.
\end{enumerate}

%\floatname{algorithm}{}
%\begin{algorithm}
%	\renewcommand{\thealgorithm}{}
%	\caption{\textbf{Proposed SDPSE}}
%	\begin{algorithmic}[1]
%		%\small
%		\State \textbf{Input:} pulse shape $p(t)$, received samples $\bm{y}$, and number of randomization iterations $Q$.
%		\State Solve $\mathcal{OP}_{\rm{SDR}}$ in \eqref{eq:opSDC}  to find $\bm{A}^*$ and $\bm{a}^*$.
%		\State Generate RV $\bm{\xi}_{q}$ as $\bm{\xi}_{q} \sim (\bm{a}^*, \bm{A}^* - \bm{a}^* \bm{a}^{*\rm{T}})$, $q = 1, ..., Q$.
%		\State Find $\breve{\bm{a}}_{q} = {\rm{sgn}}\{{\bm{\xi}}_{q}\}$.
%		\State Find $q^*  =  \arg \: \underset{q \:=\: 1, ..., Q}{\min} \quad {\breve{\bm{a}}_{q}}^{\rm{T}} \bm{G} \breve{\bm{a}}_{q} - 2 \bm{y}^{\rm{T}} \breve{\bm{a}}_{q}$.
%		\State $\hat{\bm{a}} = \breve{\bm{a}}_{q^*}$.
%		\State \textbf{Output:} estimated data symbols $\hat{\bm{a}}$.
%		%
%		%        \algstore{myalg}
%		%  \end{algorithmic}
%		%\end{algorithm}
%		%
%		%\floatname{algorithm}{}
%		%\begin{algorithm}
%		% % \ContinuedFloat
%		% \renewcommand{\thealgorithm}{}
%		%  \caption{\textbf{Proposed Algorithm} (continued)}
%		%  \begin{algorithmic}
%		%      \algrestore{myalg}
%		%     \small
%	\end{algorithmic}
%\end{algorithm}

\subsection{Complexity Discussion}
Following \cite{luo2010semidefinite}, the worst case computation complexity of the SDRSE is well-known to be polynomial time in $N$.

==> proposed.tex <==
\section{Dual Problem Solution \& Proposed Schemes} \label{sec:dual}

